The effect of mixed termination composition in Sc, Ti, and V-based MXenes

In this study, we investigate the effect of mixed surface terminations (F, O, OH) on the properties of M$_{2}$C MXenes (M = Sc, Ti, V). We explore how different compositions and patterns of terminal groups affect the stability and electronic properties of these 2D materials. The bond dissociation energies and cohesion energies show a clear preference for F-terminations in Sc$_{2}$C, while Ti- and V-based MXenes prefer O-terminations. The data indicates that terminal groups on opposite sides of the MXene have little to no influence on each other's electronic structure, allowing for independent chemical environments on each side. Semiconducting forms of studied MXenes (Sc$_{2}$CF$_{2}$, Sc$_{2}$C(OH)$_{2}$ and Ti$_{2}$CO$_{2}$) showed very high sensitivity to conduction-inducing terminations (O, O, and F, respectively) with even minuscule amounts ($\approx$1%) causing the materials to become conductive. This high sensitivity of the band gap to surface terminations may offer an explanation for the challenges in synthesizing semiconducting forms of MXenes.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
